Sequential Search with Off-Policy Reinforcement Learning

Recent years have seen a significant amount of interests in Sequential Recommendation (SR), which aims to understand and model the sequential user behaviors and the interactions between users and items over time. Surprisingly, despite the huge success Sequential Recommendation has achieved, there is little study on Sequential Search (SS), a twin learning task that takes into account a user's current and past search queries, in addition to behavior on historical query sessions. The SS learning task is even more important than the counterpart SR task for most of E-commence companies due to its much larger online serving demands as well as traffic volume. To this end, we propose a highly scalable hybrid learning model that consists of an RNN learning framework leveraging all features in short-term user-item interactions, and an attention model utilizing selected item-only features from long-term interactions. As a novel optimization step, we fit multiple short user sequences in a single RNN pass within a training batch, by solving a greedy knapsack problem on the fly. Moreover, we explore the use of off-policy reinforcement learning in multi-session personalized search ranking. Specifically, we design a pairwise Deep Deterministic Policy Gradient model that efficiently captures users' long term reward in terms of pairwise classification error. Extensive ablation experiments demonstrate significant improvement each component brings to its state-of-the-art baseline, on a variety of offline and online metrics.

==> 4-analysis.tex <==
\section{Analysis}
We look at users with long historical behavior sequence and found the DDPG model to be 

TODO: 添加类目新用户，老用户

==> DQN and DDPG in e-Commerce Search (5)/1-introduction.tex <==

\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{datasets, neural networks, gaze detection, text tagging}

%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
\begin{teaserfigure}
  \includegraphics[width=\textwidth]{sampleteaser}
  \caption{Seattle Mariners at Spring Training, 2010.}
  \Description{Enjoying the baseball game from the third-base
  seats. Ichiro Suzuki preparing to bat.}
  \label{fig:teaser}
\end{teaserfigure}

\section{Introduction}
\label{sec:introduction}

Over the past decade, neural network has seen an exponential growth in industrial applications. One of its most successful applications is in the area of search and recommendation. For instance, in the e-commerce domain, users often log onto the e-commerce platform with either vague or clear ideas of things they want to purchase. A recommender system proposes items to the user based on the items' popularity or the users' preference, inferred through past user interactions or other user profile information, while a search engine also takes into account the user provided search query as an input.

To capture a user's likely preference among the millions of items, recommendation systems have sought to leverage the user's historical interactions with the system. This is known as the Sequential Recommendation problem and has been studied thoroughly, especially after the neural network revolution in 2012, thanks to its remarkable modeling flexibility. The end result is that recommendation systems nowadays such as TikTok can deliver users' preferred content (measured in terms of post-recommendation interactions) with freakish accuracy, especially for frequent users. 

The analogous problem in the search domain, surprisingly, has been largely unexplored, at least in the published literature. Just like recommenders, search engines host billions of users. Many of these users may have interacted with the ranked results hundreds of times, through clicks in general, and also adding to cart or purchase actions in the e-commerce domain. Furthermore, unlike with recommendation systems, search engine users also leave a trail of their search queries, each of which narrows down the space of potential result candidates and can help the search engine better understand specific areas of the user's interests.

To help close this gap in the search domain, we propose a new class of learning tasks called Sequential Search. To the best of our knowledge, this is the first paper to formally introduce this new problem domain. Despite the simlarity with the well-known Sequential Recommendation problems, Sequential Search has its own sets of opportunities and challenges. First and foremost, the provision of a query in the current session significantly restricts the candidate result pool, making it feasible to approach from a ranking perspective, instead of retrieval only. At the same time, the quality of the ranked results also depends heavily on the quality of the retrieval phase. Similarly, The presence of historical queries issued by the user in principle provides much more targeted information about his or her preferences with respect to different search intents. On the flip side, however, changing queries break the continuity of the result stream presented to the user, leading to sparsity of latent ranking signals, as well as rendering personalization secondary to semantic relevance.

The present paper is an attempt to take on the aforementioned opportunities and challenges at the same time. Similar to DIEN \cite{zhou2019deep} in the Sequential Recommendation literature, we experiment with a combination of attention and RNN network to capture users' historical interactions with the system. Besides the modeling consideration stated in \cite{zhou2019deep}, such as capturing users' interest evolution, our hybrid sequential approach is also motivated by the desire to update the model incrementally during online serving, for which RNN is naturally more efficient than attention. In addition, due to the difficulty of gradient propagation over long sequences of recurrent network,  we specialize the attention component (Figure~\ref{fig:din}) to deal with long term interactions (up to 1 year) with limited number of categorical feature sequences, while apply the RNN network only to near term interactions (within the past 30 days) with the full set of features. 

Because of the multiple queries involved in the user interaction sequence, our training data takes on a special nested format (Figure~\ref{fig:user_session_tsv}) which can be viewed as a 4-dimensional array. By contrast, users in sequential recommendation problems can be treated as having a single session, albeit extended over a long period of time potentially. To further deal with the unevenness of user sequence lengths within a training minibatch, we devise a novel knapsack packing procedure to merge several short user sequences into one, thereby significantly reducing computational cost during training.

Finally to optimize for long term user experience and core business metrics, we build a deep reinforcement learning model naturally on top of the RNN framework. As is typically done, the users are treated as a partially observable environment while the recommender or search engine itself plays the role of the agent, of which the model has full control. Following ideas similar to the Deep Deterministic Policy Gradient network \cite{lillicrap2015continuous}, we introduce \textbf{S}equential \textbf{S}ession \textbf{S}earch \textbf{D}eep \textbf{D}eterministic \textbf{P}olicy \textbf{G}radient network, or S3DDPG, that optimizes a policy gradient loss and a temporal difference loss at the same time, over a continuous action space represented by the RNN output embedding as well as the agent prediction score (See Figure~\ref{fig:ddpg}). 

One difficulty in applying reinforcement learning in the search context is that the environment is essentially static. Online model exploration is expensive in terms of core business metrics, especially if the model parameters need to be explored and adjusted continuously. Fortunately our model can be trained completely offline, based only on the logged user interactions with the search results. In particular, we do not introduce any (offline) simulator component in the reinforcement learning training cycle, including the popular experience replay technique \cite{mnih2015human}. This significantly reduces model complexity compared to similar work \cite{zhao2017deep} in the Sequential Recommendation domain. Thanks to the presence of the temporal difference loss, S3DDPG also does not seem to require an adjustment of the underlying trajectory distribution, unlike the policy gradient loss only approach taken by \cite{chen2019top}.




% Deep reinforcement learning has made great breakthroughs in a variety of machine learning settings, most notably gaming, robotics. 

% More recently, it has found applications in search and recommendation ranking problems. 
% The typical setup is as follows. The users are treated as the environment, whereas the model is the player/actor. By optimizing over a long term horizon, the model seeks to induce the highest amount of reward from the users, which are typically tied to clicks or other desirable behavior, such as price-weighted purchase.  

% Unlike web search, a user on a shopping site typically interacts with the search engine multiple times before finally deciding what to buy or add to cart. This makes sequential methods such as RNN and reinforcement learning very natural candidates for behavioral predictions. 

% Despite the apparent dissimilarity, reinforcement learning is in fact supervised. Unlike ordinary setup of supervised learning in search ranking, however, reinforcement learning constructs new labels that explicitly emphasize long term rewards. This is a holy grail of well-developed e-commerce businesses, since the latter has more or less fixed pool of users, whose long term engagement and satisfaction are crucial to the sustained profitability of the business.

% One difficulty in applying reinforcement learning in the search context is that the environment is essentially static. Businesses usually cannot afford to let the model poke around the environment by intentionally trying different ranking strategies against the users. Doing so could cause severe damage to user experience, as well as require highly flexible experimentation platform to train the model continuously. 

% Thus we take an offline approach, with a similar setup to the supervised baseline. As will be discussed in Section~\ref{sec:method}, the RNN backbone is crucial for subsequent experiments in RL. We took special care to build an RNN model that is fully compatible with an earlier MLP baseline, which already includes hundreds of features of various types, such as numeric, textual, and categorical ids. In particular the training data is arranged in a contiguous and chronological order with respect to each user, so that we can treat the entire history of a user as a single example. 



% For reinforcement learning, we initially tried to follow the approach of DQN \cite{mnih2015human}. Due to the combinatorial explosion of the ranking action space, however, it quickily became clear that maximizing the Q-function over all possible ranking actions is infeasible. Instead we drop the max operator in the Bellman equation, and replace it with another objective of maximizing the discounted cumulative reward. 

% Due to the combinatorial explosion of the ranking action space, however, it quickily became clear that maximizing the Q-function over all possible ranking actions is infeasible. Instead we drop the max operator in the Bellman equation, and replace it with another objective of maximizing the discounted cumulative reward. It turns out that this is almost exactly the approach taken by Deep Determinstic Policy Gradient \cite{lillicrap2015continuous}, with several crucial differences and specializations: i) we adopt a pairwise approach for our input data, where the action consists of the representation vectors of the two chosen items; ii) Unlike most applications of RL, our reward is differentiable with respect to the action. Indeed, it is simply given by the cross entropy loss between the pairwise prediction (action) and the pairwise label.

% It is also worth noting that even though several earlier works (\cite{xu2020reinforcement}, \cite{hu2018reinforcement}) have explored the use of reinforcement learning techniques in the search ranking context, the setup has always been for a single query session, where the ranking task is decomposed into an item-by-item retrieval task. 
% Not surprisingly, we found that offline gains are disproportionate with respect to online gains in the case of RL, since factors like position bias and temporal causal effects (e.g., user will less likely click on an item purchased earlier) are not accounted in offline static evaluations. To remedy the situation, we construct an offline model for the sole purpose of simulated evaluation. This is inspired by earlier works on RL in search / recommendation, most conspicuously VirtualTaobao \cite{shi2019virtual}, as well as several search related work with open sourced implementation such as \cite{}. However the latter simulates user/ranker interactive trajectory under a single query session, whereas we look at the entire history of a user within a given training window. The use of position is also somewhat implicit in the search / recommendation related RL work. Here we make it fully explicit, by incorporating it as part of the RNN hidden state update process as well as in the simulated evaluation.

In a word, we summarize our main contributions as follows:
\begin{itemize}
    \item We formally propose the highly practical problem class of Sequential Search, and contrast it with the well-studied Sequential Recommendation.
    \item We design a novel 4d user session data format, suitable for sequential learning with multiple query sessions, as well as a knapsack algorithm to reduce wasteful RNN computation due to padding.
    \item We present an efficient combination of RNN framework leveraging all features in near-term user interactions, and attention mechanism applied to selected categorical features in the long-term.
    \item We further propose a Sequential Session Search Deep Deterministic Policy Gradient (S3DDPG) model that outperforms other supervised baselines by a large margin.
    \item We demonstrate significant improvements, both offline and online, of RNN against DNN, as well as our proposed S3DDPG against RNN, in the sequential search problem setting.
\end{itemize}


All source code used in this paper will be released for the sake of reproducibility. 
\footnote{Source code will available at https://github.com/xxxx (released upon publication)}


==> DQN and DDPG in e-Commerce Search (5)/2-related_work.tex <==
\section{Related Work}
\label{sec:related_work}


\subsection{User Behavior Modeling}
\label{subsec:rw:user}

User behavior modeling is an important topic in industrial ads, search, and recommendation system. A notable pioneering work that leverages the power of neural network is provided by Youtube Recommendation \cite{covington2016deep}. User historical interactions with the system are embedded first, and sum-pooled into fixed width input for downstream multi-layer perception. 

Follow-up work starts exploring the sequential nature of these interactions. Among these, earlier work exploits sequence models such as RNN \cite{hidasi2015session}, while later work starting with \cite{li2017neural} mostly adopts attention between the target example and user historical behavior sequence, notably DIN \cite{zhou2018deep} and KFAtt\cite{liu2020kalman}. 

More recently, self-attention \cite{kang2018self} and graph neural net \cite{wu2019session,pang2021heterogeneous} have been successfully applied in the sequential recommendation domain. 




% User Behavior Modeling Methods contains kinds of Methods:Pooling-based, Attention-based和Sequence-based。Pooling-based\cite{covington2016deep}和Attention-based\cite{zhou2018deep}, \cite{vaswani2017attention} Methods会将用户行为看成无序的集合，其中Pooling-based将所有用户行为看做是等价的。Sequence-based\cite{hidasi2015session}则可以根据用户行为序列提取信息，具有时间属性。

% ps:
% \cite{covington2016deep}: Deep Neural Networks for YouTube Recommendations.
% \cite{zhou2018deep}: Deep interest network for click-through rate prediction.
% \cite{vaswani2017attention}: Attention is all you need.
% \cite{hidasi2015session}: Session-based recommendations with recurrent neural networks.
% \label{subsec:rw:behavior}

\subsection{RNN in search and recommendation}
\label{subsec:rw:rnn}

While attention excels in training efficiency, RNN still plays a useful role in settings like incremental model training and updates. 
Compared to DNN, RNN is capable of taking the entire history of a user into account, effectively augmenting the input feature space. Furthermore, it harnesses the sequential nature of the input data efficiently, by constructing a training example at every event in the sequence, rather than only at the last event \cite{zhang2014sequential}. Since the introduction of Attention in \cite{vaswani2017attention}, however, RNN starts to lose its dominance in the sequential modeling field, mainly because of its high serving latency. 

We argue however RNN saves computation in online serving, since it propagates the user hidden state in a forward only manner, which is friendly to incremental update. In the case when user history can be as long as thousands of sessions, real time attention computation can be highly impractical, unless mitigated by some approximation strategies \cite{drachsler2008personal}. The latter introduces additional complexity and can easily lose accuracy. 

Most open-source implementations of reinforcement learning framework for search and recommendation system implicitly assume an underlying RNN backbone \cite{chen2019top}. The implementation however typically simplifies the design by only feeding a limited number of ID sequences into the RNN network \cite{zhao2019deep}. 

\cite{zhang2019deep} contains a good overview of existing RNN systems in Search / Recommendations. In particular, they are further divided into those with user identifier and those without. In the latter case, the largest unit of training example is a single session from which the user makes one or more related requests. While in the former category, a single user could come and go multiple times over a long period of time, thus providing much richer contexts to the ranker. It is the latter scenario that we focus on in this paper. To the best of our knowledge, such settings are virtually unexplored in the search ranking setting.




% RNN具备记忆能力，当涉及到连续的、与上下文相关的任务时，它比其他神经网络具有更大的优势。论文1\cite{zhang2019deep}Deep learning based recommender system: A survey and new perspectives里面将RNN在推荐系统中的应用分为三种：Session-based Recommendation without User Identifier, Sequential Recommendation with User Identifier和Feature Representation Learning with RNNs。其中不要求用户注册和登录的应用或网站没有用户标识，这些系统通常使用第一种方式通过the session或cookie获取用户的短期偏好。可以获取到用户标识的系统则使用第二种方式建模序列推荐任务，同时RNN也可作为一种特征表示的学习方式。RNN在搜索中的应用与在推荐场景中类似\cite{zhang2014sequential}。

\subsection{Deep Reinforcement Learning}
\label{subsec:rw:rl}

While the original reinforcement learning idea was proposed more than 3 decades ago, there has been a strong resurgence of interest in the past few years, thanks in part to its successful application in playing Atari games \cite{mnih2013playing}, DeepMind's AlphaGo \cite{silver2017mastering} and in text generation domains \cite{chen2019reinforcement,gong2019reinforcement}. Both lines of work achieve either super-human level or current state-of-the-art performance on a wide range of indisputable metrics.  

Several important technical milestones include Double DQN \cite{van2016deep} to mitigate over-estimation of Q value, and \cite{schaul2015prioritized}, which introduces experience replay. However, most of the work focuses on settings like gaming and robotics. We did not adopt experience replay in our work because of its large memory requirement, given the billion example scale at which we operate. 

The application in personalized search and recommendation has been more recent. Majority of the work in this area focuses on sequential recommendation such as \cite{zhao2018deep} as well as ads placement within search and recommendation results \cite{zhao2021dear}.

An interesting large scale off-policy recommendation work is presented in \cite{chen2019top} for youtube recommendation. They make heuristic correction of the policy gradient calculation to bridge the gap between on-policy and off-policy trajectory distributions. We tried it in our problem with moderate offline success, though online performance was weaker, likely because our changing user queries make the gradient adjustment less accurate.

Several notable works in search ranking include \cite{hu2018reinforcement} which takes an on-policy approach and \cite{xu2020reinforcement} which uses pairwise training examples similar to ours. However both works consider only a single query session, which is similar to the sequential recommendation setting, since the query being fixed can be treated as part of the user profile. In contrast, our work considers the user interactions on a search platform over an extended period of time, which typically consist of hundreds of different query sessions. 




% Several notable works include xyz (dawei yin, . Despite the dissimilarity between search ranking and recommendation tasks, namely the existence of a query, the problem setup is often quite similar. In particular, for learning to rank problems, typically only a single query session is considered. Many of the ranking related RL papers also focus on relevance learning, with a notable exception of xyz (Hu from alibaba). The latter however also considers a single query as the entire user history. Thus to the best of our knowledge, multi-query cross session reinforcement learniing has not been fully explored under RL.

% We also mention the work in the personalized Ads targeting domain, from ByteDance. Since it deals with the mixture of Ads and recommendation results, it does not directly address the homogeneous ranking problem that we face.


% \begin{itemize}
% \item Value-Based RL —DQN及其改进算法
% \begin{itemize}
% \item 论文1\cite{mnih2013playing}: Playing Atari with Deep Reinforcement Learning【深度强化学习开山之作】第一次提出了DQN算法，是深度强化学习真正意义的开山之作，算法用卷积神经网络构造Q网络，网络输入经过处理后的最近4帧游戏画面，输出在这种状态下执行各种动作的Q函数值。在绝大部分游戏上，DQN超过了之前最好的算法，在部分游戏上，甚至超过了人类玩家的水平；
% \item 论文2\cite{mnih2015human}: Human-level control through deep reinforcement learning 对论文1进行改进，构建目标Q网络，目标Q网络和Q网络之间周期性同步参数，提升了算法的收敛性；
% \item 论文3\cite{van2016deep}:  Deep reinforcement learning with double q-learning【Duoble DQN】 使用当前值网络的参数θ选择最优动作，用目标值网络的参数θ-评估该最优动作，将动作选择和策略评估分离，降低了过高估计Q值的风险；
% \item 论文4\cite{schaul2015prioritized}: Prioritized experience replay【Prioritized replay 样本采样方式优化】基于优先级采样的DQN，是对经验回放机制的改进，为经验池中的每个样本计算优先级，增大有价值的训练样本在采样时的概率。加快收敛速度和提升效果；
% \item 论文5\cite{wang2016dueling}: Dueling network architectures for deep reinforcement learning【Dueling networks】将CNN卷积层之后的全连接层替换为两个分支，其中一个分支拟合状态价值(state values)函数V(s)，另外一个分支拟合动作优势(action advantages)函数A(s,a)。最后将两个分支的输出值相加，形成Q函数值。这种改进能够更准确的估计Q值。
% \item 论文6\cite{hausknecht2015deep}:Deep recurrent q-learning for partially observable MDPs. 在CNN的卷积层之后加入LSTM单元，记住之前的信息。
% \item 论文7\cite{hessel2018rainbow}: Rainbow: Combining Improvements in Deep Reinforcement Learning 整合了DQN的诸多优化。包括Double Q-learning，Prioritized replay，Dueling networks，Multi-step learning，Distributional RL 和 Noisy Nets.
% \item DQN适用范围：DQN是求每个action的\(max_aQ(s,a)\)，适用于低维，离线的动作空间，在连续空间不适用。
% \end{itemize}
% \item Policy-Based RL算法
% \begin{itemize}
% \item  policy based RL 直接对策略建模，通过reward来直接对策略进行更新，使得累计回报最大。适用于连续的动作空间，但是无法衡量策略究竟是不是最优，策略评估高方差。
% \item  最开始的reinforcement算法\cite{williams1992simple} Simple Statistical Gradient-Following Algorithms for Connectionist Reinforcement Learning[1992, Williams] 
% \item  策略梯度算法\cite{sutton1999policy} Policy Gradient Methods for Reinforcement Learning with Function Approximation[2000, Sutton]
% \end{itemize}

% \item Actor-Critic算法
% \begin{itemize}
% \item 结合Policy-Based RL和Value-Based RL方法，基本上解决了高维状态与动作空间的问题，并使性能有明显的提升。但原始的Actor-Critic方法对于复杂问题可能会不稳定。
% \item DPG算法\cite{silver2014deterministic}：Deterministic Policy Gradient Algorithms【DPG】
% \item DDPG算法\cite{lillicrap2015continuous}：Continuous Control With Deep Reinforcement Learning【DDPG】
% \item TD3算法\cite{fujimoto2018addressing}：Addressing Function Approximation Error in Actor-Critic Methods【Twin Delayed Deep Deterministic policy gradient TD3】
% \end{itemize}

% \end{itemize}

% \label{subsec:rw:rl}

% \subsection{Reinforcement Learning in search and recommendation、}
% \begin{itemize}
% \item 传统的搜索/推荐算法
% \begin{itemize}
% \item 认为搜索/推荐是一个静态的过程；
% \item 建模即时reward，仅考虑当前的商品是否被点击/购买，忽略长期价值；
% \end{itemize}
% \item 强化学习在推荐中的应用
% \begin{itemize}
% \item  MDP推荐系统\cite{shani2005mdp}：An MDP-Based Recommender System
% \item  RL推荐系统（最大化长期价值）\cite{theocharous2015ad}：Personalized ad recommendation systems for life-time value optimization with guarantees
% \begin{itemize}
% \item 把个性化⼴告推荐系统定义为强化学习问题，最⼤化⽣命周期值(life-time value)
% \end{itemize}
% \item  DRN新闻推荐\cite{zheng2018drn}:DRN:A deep reinforcement learning framework for news recommendation
% \begin{itemize}
% \item 基于【DQN】的推荐算法
% \item 主要贡献：1.提出基于deep Q-learning的推荐框架，该框架可以明确建模长期reward（MAB-based方法不更清晰地给出future reward,MDP-based方法不适用于大规模数据）；2.引入用户活跃度（用户返回APP的情况），作为点击/不点击标签的补充，从而获取更多的的用户反馈信息；3.加入了探索策略（采用Dueling Bandit Gradient Descent方法挑选当前推荐环境下候选items），为用户寻找新的有吸引力的新闻；
% \end{itemize}
% \item Listwise推荐\cite{zhao2017deep}：Deep reinforcement learning for list-wise recommendations
% \begin{itemize}
% \item 基于【DDPG】的推荐算法
% \item 主要缺点：使用全联接网络表示用户状态，不能很好的建模用户和商品之间的关系
% \end{itemize}
% \item Pagewise推荐\cite{zhao2018deep}：Deep Reinforcement Learning for Page-wise Recommendations
% \begin{itemize}
% \item 基于【DDPG】的推荐算法
% \item 主要贡献：生成每个推荐物品的同时，也决定每个推荐维度在二维屏幕上的位置
% \end{itemize}
% \item 考虑正负反馈的推荐\cite{zhao2018recommendations}：Recommendations with Negative Feedback via
% Pairwise Deep Reinforcement Learning
% \begin{itemize}
% \item 基于【DQN】的推荐算法
% \item 主要贡献：考虑负反馈以及商品的偏序关系，并将这种偏序关系建模到DQN的loss函数中。用户跳过或者是没有任何行为的商品，不仅能够影响用户的行为，还可以让我们更好的了解用户的偏好。
% \end{itemize}
% \item User-Item Interactions Modeling\cite{liu2018deep} : Deep Reinforcement Learning based Recommendation with Explicit User-Item Interactions Modeling
% \begin{itemize}
% \item 基于【DDPG】的推荐算法
% \item 主要贡献：状态表征模块设计，文中强调了状态表征的重要性，并设计了三种状态表征模块；DRR-p：商品之间组pair，pair内item embedding相乘，和原始商品信息concat；DRR-u：用户embedding和item embedding相乘，同时concat商品pair相乘结果；DRR-ave：DRR-u基础上item处考虑position weight，并经过average pooling；
% \item 不足之处：虽然设计了状态表征模块，但是仅使用了用户最近的N个正反馈商品
% \end{itemize}
% \end{itemize}

% \item 强化学习在搜索中的应用
% \begin{itemize}
% \item 阿里RL搜索排序\cite{hu2018reinforcement}：Reinforcement learning to rank in e-commerce search engine: Formalization, analysis, and application
% \end{itemize}

% \end{itemize}

\label{subsec:rw:rl_search}

% mainly low rank approximation and pq based.


==> DQN and DDPG in e-Commerce Search (5)/3-method.tex <==
\section{Method}
\label{sec:method}
We introduce the main model architecture in this section. Each subsection forms the foundation for the next one. Section~\ref{sec:din} describes an attention based network inspired by \cite{zhou2018deep} that exploits the correlation between the current ranking task and the entire historical sequence of items for which the user has expressed interest. Section~\ref{sec:rnn} details an elaborate Recurrent Neural Net backbone that can efficiently handle a batch of uneven sized sequences, and how it is used to capture more recent user interactions with the search engine. The output embedding of the attention network is simply fed as an input into every timestamp of the recurrence. Finally we discuss how to build an actor-critic style reinforcement learning model on top of the RNN structure in section~\ref{sec:ddpg}. 

\subsection{Attention for Long-Term Session Sequence}
\label{sec:din}
As mentioned in section~\ref{subsec:rw:user}, the attention network in the Deep Interest Network (DIN) model is a natural way to incorporate user history into personalized recommendation. To adapt to the search ranking setting, we introduce Search Ranking Deep Interest Network (DIN-S), which makes the following adjustments on top of DIN:
\begin{itemize}
    \item Query side features are introduced alongside the focus item features, to participate in attention with historical item sequence.
    \item To account for the possibility that the current query request is not correlated with any of the user's past actioins, a zero score is appended to the regular attention scores before getting the softmax weights. This is illustrated by the zero attention unit in Figure~\ref{fig:din}.
\end{itemize}https://www.overleaf.com/project/5fed74e5fac2600586cb62da
% The only difference in personalized search is to add query related features to the attend list. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DIN.png}
    \centering
    \caption{DIN-S architecture.}
    \label{fig:din}
\vspace{-5pt}
\end{figure}

The overall architecture of DIN-S is outlined in Diagram~\ref{fig:din}. Due to the nature of algorithmic iterations within an industrial setting, DIN-S is not only one of our quality comparison baselines, but also one of the major components in our proposed final architecture.
We have also tried DIEN \cite{zhou2019deep} and other follow up works. Despite the better results reported in papers, we found little incremental improvement in our own systems. However our design of the RNN backbone model shares some similarity with the approach in DIEN, and indeed both ours and the DIEN work use attention and RNN together. A key difference, however, is that our RNN training data and algorithmic design uses all features available in previous interactions by the user, including both item or query/user one-sided as well as two-sided features. By contrast, the RNN (GRU) in DIEN appears to be just an extension of the co-existing Attention network, taking mostly item-side only categorical features.

\subsection{RNN for Near-Term Sequential Search}
\label{sec:rnn}
In order to compare with the baseline DIN-S (attention + MLP) model fairly and conveniently, we build a so-called RNN backbone that can wrap around any base model architecture. The logic is outline in the bottom half of Diagram~\ref{fig:rnn}. To summarize, for any base model $M$, the RNN backbone introduces a new feature vector $H_t$, the hidden state, concatenated to the output of $M$. The output of each time iteration of the RNN model is another vector $H_{t+1}$, which serves both as the input to downstream networks, as well as the hidden state input for the next time iteration. 

\subsubsection{Contiguous Session-Based Data Format}
\label{subsubsec:data_format}
While DIN-S can be trained in a pointwise / pairwise fashion, our implementation of RNN tries to pool all relevant information together in the data by 
\begin{itemize}
    \item arranging all items within a query session in a single training example. In our case we used tsv (tab-separated values) format. Thus the number of columns in each row is variable, depending on the number of items under the session.
    \item placing all query sessions belonging to the same user contiguously to ensure they are loaded altogether in a mini-match.
\end{itemize}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DDPG-UserSessionTSV.png}
    \centering
    \caption{User Session Input Format. $B$ stands for batch size. Each row represents a single TSV row in the input data. The numbers of columns = number of query features + num of items $\times$ number of item features.}
    \label{fig:user_session_tsv}
\vspace{-5pt}
\end{figure}
As illustrated in Figure~\ref{fig:user_session_tsv}, each mini-batch thus contains a 4d tensor $B$ whose elements are indexed by $(u, t, i, f)$, which stand for users, sessions (time-ordered), items, and features respectively. We assume that features are all dense or have been converted to fixed width dense format, through either embedding sum-pooling or 
attention-pooling from the DIN-S base model. We will use $B_{u, t}$ to denote the 2d slices of $B$ containing all $(i, f)$ values. 
% \vspace{-20pt}

\subsubsection{RNN Model Architecture}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{RNN.png}
    \centering
    \caption{RNN architecture.}
    \label{fig:rnn}
\end{figure}
Let $\omega_{u, t}, H_{u, t}$ stand for the regular output and hidden state output of the RNN network for user $u$ and session $t$. The RNN network can thus be described by a function $F$ with the following signature
\begin{align} \label{eq:rnn_kernel}
    (\omega_{u, t+1}, H_{u, t+1}) = F(B_{u, t + 1}, H_t).
\end{align}
This is the most general form of an RNN network. All RNN variants such as LSTM, GRU obey the above signature of $F$.

Recall now $B_{u, t}$ is a 2d tensor, with dimension given by (the number of items, number of features). The same is true of the output tensor $\omega_{u,t}$. The hidden state $H_{u, t}$ however has \textbf{no item dimension}: it is a fixed width vector for a given user after a given session. For simplicity, our choice of $F$ simply computes $H_{u, t}$ as a weighted average of the output $\omega_{u, t}$. More precisely,
\begin{align}
    \omega_{u, t+1}, S_{u, t+1} &= \rm{GRU}(\omega_{u, t}, S_{u, t}) \\
    H_{u, t+1, f} &= \frac{1}{|\cC_{u, t}|} \sum_{j \in \cC_{u, t}} \omega_{u, t+1, j, f}. 
\end{align}
Here $\cC_{u, t}$ stands for the set of items in user $u$'s session $t$ that were purchased. Those sessions without purchases are excluded from our training set, since under the above framework, 
\begin{enumerate}
    \item the user hidden state would not be updated;
    \item the final pairwise training label contains no information.
\end{enumerate} 
The vast majority of the remaining sessions contain exactly 1 purchased item.

This completes the description of the RNN evolution of the state vector under a listwise input format, where all items in a session are used. For training efficiency, however, we adopt a pairwise setup, where 2 items are sampled from each query session, and exactly one of them has been purchased. Thus we can think of each session as consisting of exactly 2 items. Since the hidden state is a weighted average over only the purchased items, pairwise sampling preserves all the information for the hidden state vector in a single RNN step, provided the session contains only a single purchased item, which is more than $90\%$ of the cases.

Lastly, the RNN model outputs a single logit $\eta_{u, t, i}$ for each item $i$ chosen within the user session $(u, t)$, by passing the RNN output vector $\omega_{u, t, i} \in \R^d$ of dimension $d$ through a multi-layer perception $P$ of dimensions $[1024, 256, 64, 1]$:
\begin{align} \label{eq:rnn_output}
    \eta_{u, t, i} = P(O(u, t, i)),  \quad P: \R^d \to \R.
\end{align}
The corresponding label is a binary indicator $\lambda_{u, t, i} \in \{1, 0\}$, which denotes whether the item was purchased or not.

\subsubsection{Pairwise Loss} \label{subsec:rnn:pairwise}
Unlike clicks or mouse hover actions, each page session in e-commerce search typically receives at most one \textbf{purchase}. Thus we are confronted with severe positive and negative label imbalance. To address this problem, we choose pairwise loss in our modeling, which samples a purchased item from the current session at random, and matches it with a random item that is viewed or clicked but not purchased. 

The exact sampling procedure is described in Algorithm~\ref{alg:pairwise_sampling}. Note that as long as the session is non-empty, the procedure will always output a pair. There are occasional edge cases when all items are purchased, in which case we output two purchased items. Alternatively, such perfect sessions can be filtered from the training set.

\begin{algorithm}[t]
\caption{Pairwise sampling from a query session.}
\label{alg:pairwise_sampling}
\begin{algorithmic}[1]
\REQUIRE{a list of $N > 0$ labels: $\lambda_1, \ldots, \lambda_N \in \{0, 1\}$}
\ENSURE{two indices $1 \leq a, b \leq N$, s.t. $\lambda_a = \max \lambda_i$ and $\lambda_b = \min \lambda_i$}
\STATE Compute $\lambda_{\min} := \min_i \lambda_i$ and $\lambda_{\max} := \max_i \lambda_i$.
\STATE Construct the list of admissible pairs $A := \{(a, b) \in [N]^2: \lambda_a = \lambda_{\max}, \lambda_b = \lambda_{\min}\}$ 
\STATE Output a uniformly random element $(a, b)$ from $A$.
\end{algorithmic}
\end{algorithm}
% Our choice of pairwise loss is motivated by the disparity between positive and negative examples within each session: typically users only make a single purchase out of a page of 10 results. 
The final loss function on an input session $(u, t)$ is given by the following standard sigmoid cross entropy formula:

\begin{align} \label{eq:logloss}
    &\cL(B_{u, t}, \lambda_{u, t}) = -\lambda_{u, t} \log \sigma(\eta_{u, t}) - (1-\lambda_{u, t}) \log (1 - \sigma(\eta_{u, t}))
\end{align}
where 
\begin{itemize}
\item $B_{u, t}$ stands for all the features available to the model for a given user session $(u, t)$.
\item $\lambda_{u, t} := \lambda_{u, t, a, b} = \frac{\lambda_{u, t, a}}{\lambda_{u, t, a} + \lambda_{u, t, b}} \in \{0, 1\}$, depending on whether a purchase was made on item $a$ or $b$ within the user session $(u, t)$. 
\item $\eta_{u, t} := \eta_{u, t, a, b} = \eta_{u, t, a} - \eta_{u, t, b}$ is simply the difference between the model outputs for the two items $a$ and $b$, which can be interpreted as the log-odds that the purchase was made on the first item.
\item $a, b$ are a pair of random item indices within the current session, chosen according to Algorithm~\ref{alg:pairwise_sampling}, where item $a$ is purchased while item $b$ is not.
\item $\sigma(\eta_{u, t})$ transforms the pairwise logit $\eta_{u, t}$ through the sigmoid function $\sigma: x \mapsto (1 + e^{-x})^{-1}$, and can be interpreted as the model predicted probability that item $a$ is purchased, given exactly one of item $a$ and $b$ is purchased.
\end{itemize}

% \\
%     &\frac{\ell_{u, t, i}}{\ell_{u, t, i} + \ell_{u, t, j}} \log \frac{e_{u, t, i}}{e_{u, t, i} + e_{u, t, j}} + \frac{\ell_{u, t, j}}{\ell_{u, t, i} + \ell_{u, t, j}} \log \frac{e_{u, t, j}}{e_{u, t, i} + e_{u, t, j}}
\subsubsection{Knapsack Sequence Packing}
Since the numbers of historical sessions vary widely across different users, the naive implementation of the above 4d representation can be computationally quite wasteful due to excessive zero padding. We thus adopt a knapsack strategy (Algorithm~\ref{alg:knapsack_rnn}) to fit multiple short user session sequences into the maximum length seen in the current mini-batch. 

\begin{algorithm}[t]
\caption{Parallel RNN via Knapsack Packing}
\label{alg:knapsack_rnn}
\begin{algorithmic}[1]
\REQUIRE{a list of $N$ (user, session) indices: $\cI = \{(u_1, 1), \ldots, (u_1, T_1), \ldots, (u_n, T_n)\}$}
\REQUIRE{input feature vectors associated with each (user, session) pair: $\{B_{u, t} \in \R^D: (u, t) \in \cI\}$}
\REQUIRE{an expensive RNN kernel $\tilde{O}: \R^{2D} \to \R^{2D}$}
\ENSURE{efficient computation of $\{\omega_{u, t} := O(B_{u, t}): (u, t) \in \cI\}$}
\STATE Apply the greedy knapsack strategy (Algorithm~\ref{alg:greedy_knapsack}) to get a mapping $m: (u, t) \mapsto (u', t')$, as well as the 2d array $S := \{S_{u', t'}\}$ that encodes the starting positions of the subsequences.
\STATE Construct a new input features $B'$ according to $B'_{u', t'} = B_{u, t}$.
\STATE Zero pad the missing entries of $B'$, for vectorized processing.
\STATE Compute $\omega' := O'(B', S)$ for all packed users in parallel.
\STATE Rerrange $\omega'_{u', t'}$ into the original user sequences $\omega_{u, t}$ via the inverse map $m^{-1}: (u', t') \mapsto (u, t)$.
\end{algorithmic}
\end{algorithm}
To break down Algorithm~\ref{alg:knapsack_rnn}, we introduce a few terminologies:
\begin{definition}
For a given RNN kernel $\tilde{O}: \R^D \times \R^D \to \R^D \times \R^D$, its associated \textbf{sequence map} $O: \R^{D \times T} \to \R^{D \times T}$, $(B_1, \ldots, B_T) \mapsto (\omega_1, \ldots, \omega_T)$ is given inductively by 
\begin{align*}
    (\omega_1, H_{u, 1}) &:= \tilde{O}(B_{u, 0}, H_{u, 0}) \\
    (\omega_{t+1}, H_{u, t+1})  &:= \tilde{O}(\omega_t, H_{u, t}) \quad \text{for } t \leq T -1.
\end{align*}
The initial hidden state is typically chosen to be the all zero vector: $H_{u, 0} = \vec{0}$.
\end{definition}

Note that after applying the knapsack packing Algorithm~\ref{alg:greedy_knapsack}, the maximum length of all the sequences stays the same. The total number of sequences, however, is reduced, by an average factor of 20x. As a result, some new sequence now contains multiple old sequences, arranged contiguously from the left. In such cases, we do not want the hidden states to propagate across sequences. Thus we introduce the following extended RNN sequence map that takes into account the old sequence boundary information:
\begin{definition}
Given an RNN kernel $\tilde{O}$ as above, and a 2d indicator array $\{S_t \in \{0, 1\}: 1 \leq t \leq T\}$ denoting the starting positions of sub-sequences within each user sequence, the \textbf{boundary-aware sequence map} 
\begin{align*}
    O': \R^{D \times T} \times  \{0, 1\}^{D \times T} \to \R^{D \times T}, \quad (B_1, \ldots, B_T) \mapsto (\omega_1, \ldots, \omega_T)
\end{align*} 
is defined via the following inductive formula
\begin{align*}
    (\omega_1, H_{u, 1}) &:= \tilde{O}(B_{u, 0}, H_{u, 0}) \\
    (\omega_{t + 1}, H_{u, t + 1}) &:= 
    \begin{cases}
      \tilde{O}(B_{u, t}, H_{u, 0}) & \text{if  $S_{t+1} = 1$ }\\
      \tilde{O}(\omega_t, H_{u, t}) & \text{otherwise}
    \end{cases}  
\end{align*}
\end{definition}
 
% TODO(jyj): check table stats to ensure logical soundness here.
% The numbers of items per session typically do not vary by much, and have a mean around 10; indeed we count users' next page request under the same query as a separate session. Thus there is little marginal benefit to apply knapsack packing along the item dimension. Furthermore, under the pairwise training strategy (Section~\ref{subsec:rnn:pairwise}, each session consists of exactly 2 items, making the item dimension already uniform across sessions. 

Overall the session knapsack strategy saves about 20x compute and speed up CPU training time by about 3x. Note that during online serving, knapsack is not needed since we deal with one user at a time.
\begin{algorithm}[t]
\caption{Greedy Knapsack Sequence Packing.}
\label{alg:greedy_knapsack}
\begin{algorithmic}[1]
\REQUIRE{A nonempty index set $\cI := \{(u_1, 1), \ldots, (u_1, T_1), \ldots, (u_n, T_n)\}$.}
\ENSURE{an index map $m: \cI \to \cU' \times [T']$, where $|\cU'| \leq n$ is the packed user index set and $T' \leq \max_i T_i$.}
\ENSURE{a 2d array $S_{u', t'}$ indicating the start positions of subsequences in each packed user sequence.}  
\STATE Set $T' := \max_{i=1}^n T_i$.
\STATE Initialize $U := [n] \setminus \{i\}$.
\STATE Initialize the list of knapsacks $\cK \leftarrow []$.
\STATE Initialize $S_{u', t'}$ to the all $0$ 2d array.
\WHILE {$U \neq \emptyset$}
    \STATE Pop a longest user sequence from $U$, say $u_j$.
    \IF {$T_j + \sum_{k \in \cK_i} T_k < T'$ for some $i \leq |\cK|$}
        \STATE Define $m(j, \ell) := (i, \ell + \sum_{k \in \cK_i} T_k)$ for $\ell < T_j$.
        \STATE Set $S_{i, \sum_{k \in \cK_i} T_k} \leftarrow 1$.
        \STATE Append $j$ to the end of $K_i$.
    \ELSE
        \STATE Append $[j]$ to the end of $\cK$.
        \STATE Define $m(j, \ell) := (|\cK|, \ell)$
        \STATE Set $S_{|\cK|, 1} \leftarrow 1$.
    \ENDIF
\ENDWHILE

\end{algorithmic}
\end{algorithm}
\subsection{DDPG for Near-Term Future Sessions}
\label{sec:ddpg}

While attention and RNN are capable of leveraging past sequential data, they fall short of predicting or optimizing future user behavior several steps in advance. This is not surprising because the former are essentially trained in a supervised approach, where the target is simply the next session. To optimize trajectories of several future sessions, we naturally turn to the vast repertoire of reinforcement learning (RL) techniques. 

As mentioned in Section~\ref{subsec:rw:rnn}, unlike the vast majority of RL literature in search and recommendation, our trajectory of agent (ranker) / environment (user) interaction is not confined within a single query session. Instead the user continues to type new queries, over a span of weeks or months. Thus the environment changes from one session to the next. However a key assumption here is that the different manifestations of the environment (user) share an underlying preference theme, as a single user's shopping tastes are strongly correlated across multiple shopping categories or intents.

Another important difference between our sequential session setup and the single session setup in other works is that each step of S3DDPG needs to rank a list of tens or hundreds of items, rather than just picking the top K from the remaining candidate pool. Due to the combinatorial explosion associated with ranking tasks, it becomes infeasible to treat the set of permutations of the items as our action space. Instead we take the vector output of the RNN network, along with the actor network prediction, as the action, which lives in a continuous space.
% Table~\ref{tab:modeling_differences} summarizes the key areas where S3DDPG departs from existing RL work in search and recommendation.

% \begin{table}[htbp]
% \centering
% \caption{Modeling Difference}
% \small
% \begin{tabular}{c|c|c}
% \hline
% Key Areas & Our Work & Typical Other Work \\
% \hline
% Single Step Task & \begin{tabular}{@{}c@{}}Independent \\ Ranking\end{tabular} & \begin{tabular}{@{}c@{}} Masked Top-K \\ Retrieval \end{tabular} \\
% \hline
% Explicit Actions & 10! permutations & Candidate Items \\
% \hline
% Implicit Actions & RNN output vector & Candidate Items \\
% \hline
% \begin{tabular}{@{}c@{}} Environment \\
% (User Intent) \end{tabular} & Dynamic & Static \\
% \hline
% \end{tabular}
% \label{tab:modeling_differences}
% \end{table}


\subsubsection{S3DDPG Network}

\begin{figure}
    \centering
    % \includegraphics[width=\linewidth]{DDPG.png}
    \includegraphics[scale=0.5]{ddpg_new.png}
    \centering
    \caption{S3DDPG architecture.}
    \label{fig:ddpg}
\end{figure}

Finally we come to our reinforcement-learning based ranking framework, which is depicted in Diagram~\ref{fig:ddpg}. The bottom half of the network consists of the RNN structure described in the previous subsection. The reinforcement learning part takes the regular RNN output (i.e., non-hidden state related) as the input, and is similar to the actor/critic framework. We closely follow the logic of DDPG network \cite{lillicrap2015continuous}.

The actor network has the same structure as the final MLP layers in RNN that takes the intermediate embedding to per-item logit. The latter is thus used also as the final ranking score for each item within a single query session. 

The critic network (also known as the Q-network) is a separate multi-layer perceptron, $Q: \R^d \to \R$, taking \textbf{a pair of RNN outputs} $\omega_{u, t, a}, \omega_{u, t, b} \in \R^d$ to a single scalar logit. 
\begin{align*}
    q_{u, t} := Q(\omega_{u, t, a}, \omega_{u, t, b}) \in \R.
\end{align*}

$Q$ is introduced here to approximate the following maximal cumulative discounted long term reward:
\begin{align*}
    q_{u, t} \sim \sup_{\eta_{u, t}, \ldots, \eta_{u, T}} \sum_{s = t}^T \gamma^{s - t} r(\eta_{u,  t}, \lambda_{u, t}).
\end{align*}

Here the supremum is taken over all trajectories starting at session $t$, and the reward $r(\eta_{u,t},\lambda_{u, t}) =: r_{u, t}$ is simply given by the opposite of the sigmoid cross entropy loss $\cL(B_{u, t}, \lambda)$ (See \eqref{eq:logloss}):
% reproduced here for convenience:
\begin{align} \label{eq:reward_definition}
    r(\eta_{u, t}, \lambda_{u, t}) = \lambda_{u, t} \log \sigma(\eta_{u, t}) + (1 - \lambda_{u, t}) \log \sigma(1 - \eta_{u, t}).
\end{align}
The time horizon $T$ itself is also random in general.

To summarize, we have introduced three networks and their associated output layers so far
\begin{itemize}
    \item $\omega_{u, t, a}, \omega_{u, t, b} \in \R^d$ are the output vectors of the RNN network for the chosen item pair.
    \item $\eta_{u, t} = P(\omega_{u, t, a}) - P(\omega_{u, t, b})$ is the scalar output of the actor network, which has the interpretation of log-odds of the first item being purchased.
    \item $q_{u, t} = Q(\omega_{u, t, a}, \omega_{u, t, b})$ is the scalar output of the critic (Q) network for the pair.
\end{itemize}


The critic (Q) network differs significantly from the actor network $P$ in that the input consists of pairs of items. Thus unlike $\eta_{u, t}$, it is not anti-symmetric under swapping of the item pair.


It is interesting to note that the original supervised loss function $\cL(\eta, \lambda)$ has been re-purposed as the reward in the Q-network. The actual loss functions are defined next.
% At this stage, we have not defined the loss function of our S3DDPG model yet, which we proceed to do next.

\subsubsection{Loss Functions}
There are two loss functions in the S3DDPG framework. The first of these two, the temporal difference (TD) loss, is well-known since the first DQN paper \cite{mnih2013playing}. It aims to enforce the Bellman's equation on the Q-values:
\begin{align} \label{eq:bellman}
    q_{u, t} = \sup_{\eta_{u, t}} r(\eta_{u, t}, \lambda_{u, t}) + \gamma q_{u, t + 1}.
\end{align}
Here $\gamma$ is a discount factor, which is set to $0.8$ throughout our experiments. The associated TD loss would then be
\begin{align} \label{eq:dqn_td_loss}
    \cL^{\text{DQN}}_{\text{TD}} (B_{u, t}, \lambda_{u, t}) := \sum_{u \in \cU} \sum_{t=1}^{T - 1} (q_{u, t} - \sup_\eta \left\{r_t(\eta, \lambda) - \gamma q_{u, t+1}\right\})^2.
\end{align}
Here $\cU$ stands for all the users in the training data, and $T$ implicitly depends on the choice of $u$. 

% As mentioned in Table~\ref{tab:modeling_differences}, however,
As mentioned in Section~\ref{sec:ddpg}, however, our action space is either combinatorially explosive ($10!$), or continuous $\R^d$. Thus it is unclear how to compute the supremum on the right hand side. Instead we simply drop the supremum operator and consider the following weakened Bellman equation
\begin{align} \label{eq:weak_bellman}
    q_{u, t} = r(\eta_{u, t}, \lambda_{u, t}) + \gamma q_{u, t + 1}, \quad q_{u, T} = 0.
\end{align}
The TD loss thus aims to minimize the sum-of-square error between the two sides of the equation above:
\begin{align} \label{eq:td_loss}
    \cL_{\text{TD}}(B_{u, t}, \lambda_{u, t}) := \sum_{u \in \cU} \sum_{t=1}^{T - 1} (q_{u, t} - r_{u, t} - \gamma q_{u, t + 1})^2.
\end{align}
The problem with the above weakened TD loss \eqref{eq:td_loss} is that by itself, it is under-specified. Indeed, $r_{u, t} = r(\eta_{u, t}, \lambda_{u, t})$ can take on any (negative) value without affecting $\cL_{\text{TD}}$, since the extra degrees of freedom in $q_{u, t}$ can easily compensate for its wild moves. By contrast, the original TD Loss (for DQN) \eqref{eq:dqn_td_loss} eliminates this extra degree of freedom by taking the supremum over all actions $\eta_{u, t}$. 

To make the training loss fully specified, we thus introduce a second loss term, the policy gradient (PG) loss, which seeks to maximize the cumulative Q-value over the RNN and critic network model parameters. 
\begin{align}
    \cL_{\text{PG}}(B_{u, t}, \lambda_{u, t}) := \sum_{u \in \cU} \sum_{t=1}^T q_{u, t}, \quad q_{u, t} = Q(O(B_{u, t})).
\end{align}
where recall $q_{u, t} = Q(O(B_{u, t, a}), O(B_{u, t, b}))$ for the chosen positive / negative item pair. Note that since the actor network also depends on the RNN network parameters, the PG loss also indirectly optimizes over the action space. Furthermore, since $q_{u, t}$ are very closely tied with the supervised reward function $r_t$, by maximizing $q_{u, t}$, we are implicitly also maximizing the original supervised reward.


% This prediction is then fed into a policy gradient loss, which takes into account the logged user feedback label, which in our case is the binary signal of whether the current item has been purchased. The exact policy gradient loss is given by the formula below
% \begin{align}
%     \rm{PGLoss} = \sum_{t=1}^T \gamma^t \mathbb{E} Q_t, \quad Q_t := Q(\omega_{u, t}, P_{u, t}) 
% \end{align}

% The critic network takes the RNN output and actor output (the scalar logit value) as its input, and tries to simulate the Q value associated with the Bellman equation, which is a vector, $\{Q_t: 1 \leq t \leq T\}$, indexed by the session ids. The resulting Q value output is then used to compute a temporal difference loss which measures the deviation from the exact Bellman equation.
% \begin{align}
%     \rm{TDLoss} = \sum_{t=1}^{T-1} (Q_t - \gamma Q_{t+1} - r_t)^2.
% \end{align}

As is standard in DQN and DDPG, we also add the so-called target Q-network \cite{mnih2015human}, denoted by $\tilde{Q}$, that differs from the original Q-network only by one time-step, which is useful for stabilizing its learning. In other words, the exact weight updates are given by,
\begin{align}
    Q &\leftarrow Q + \alpha \nabla_Q (\sum_{t = 1}^{T - 1} Q(\omega_t) - \gamma \tilde{Q}(\omega_{t+1}) - r_t) \\
    \tilde{Q} &\leftarrow Q ,
\end{align}
where $\alpha$ is the effective learning rate that depends on the actual 1st order optimizer used.


% TODOs:
% 1. Put a formula about target Q-network here.
% 2. Put a formula about GRU here.
% 3. Put a formula about 


% One distinguishing feature of DDPG from DQN is that besides Q-learning, there is also policy learning, expressed through the policy gradient loss. The latter tries to maximizes the expected discounted cumulative reward over available actions given the current state. This is naturally done through gradient descent in our ranking problem since the parameter space is continuous, where exact discrete maximization is highly infeasible.
% Due to the instability of optimizing both the target and the source in Q loss, we use two copies of the Q network, and periodically copy the source version (at $t$) to the target (at $t + 1$).

We have also tried two versions of the actor networks, but the difference in evaluation metrics is small (about 0.04\% in session AUC), thus was discarded for simplicity and training efficiency.

Another important way S3DDPG differs from traditional DDPG implmementation is the relation between the two losses and weight updates. In the original proposal \cite{lillicrap2015continuous}, the actor and critic network weights are updated separately by the PG and TD losses:
\begin{align*}
    P \leftarrow P + \alpha \nabla_P \cL_{\text{PG}}, \qquad Q \leftarrow Q + \alpha \nabla_Q \cL_{\text{TD}}.
\end{align*}
However we cannot get the model to converge under this gradient update schedule. Instead we simply take the sum of the two losses $\cL_{\text{PG}} + \cL_{\text{TD}}$, and update all the network weights according to
\begin{align*}
    O, P, Q \leftarrow \alpha \nabla_{O, P, Q} (\cL_{\text{PG}} + \cL_{\text{TD}}).
\end{align*}


\section{Online Incremental Update}
To capitalize on the underlying RNN modeling framework, we perform incremental update when the model is served online, so that the most recent user interactions can be captured by the model to update the user states. The overall architecture and its relation to offline training is summarized in Figure~\ref{fig:incremental_update}. The offline trained model can be divided into two sets of network parameters: 
\begin{itemize}
    \item The user state aggregation network takes the hidden states associated with all the items in the session, along with their corresponding labels, and perform average pooling to obtain a fixed size updated user state. If the session contains no purchase action, we do not update the user state.
    \item The remaining network take in the usual input features, along with the user state, to output predictions for each item.
\end{itemize}
The first of these is sent to an online incremental update component. While the latter goes directly to the neural network scorer.

The online serving component is roughly divided into three modules. At the center is the search engine itself, which is in charge of distributing and receiving features. 

When a user types in a query, the associated user context features, including query text, user's basic profile information, as well as user's historical actions, are all sent to the search engine. The search engine then relays this information to the neural network predictor, which in turn computes the predicted scores as well as the hidden state for each item, all of which are sent back to the search engine. Finally if the user makes any purchase in the current session, the new user state is updated to be the average of hidden states from the purchase items. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{DDPG-IncrementalUpdate.png}
    \caption{Real-Time Incremental Update Pipeline.}
    \label{fig:incremental_update}
\vspace{10pt}
\end{figure}

% TODOs:
% 1. add some diversity time series plot.
% 2. add UV value time series plot.
% 3. show some arena side by side to show diversity.
% 4. 


==> DQN and DDPG in e-Commerce Search (5)/4-analysis.tex <==
\section{Analysis}
We look at users with long historical behavior sequence and found the DDPG model to be 

TODO: 添加类目新用户，老用户

==> DQN and DDPG in e-Commerce Search (5)/5-experiment.tex <==
\section{Experiment}
\label{sec:experiment}
\subsection{Evaluation Setup}
% \subsection{Setup}
% \label{sec:setup}
% Our primary evaluation is carried out on an in-house dataset collected from the 1 month of search log. This has the advantage of being 
% % We used one industrial scale in-house dataset and one public Amazon review dataset. The former has the advantage of being 
% directly reflected in online experiments, which is the most important way to validate our idea in an industrial setting. 
% The latter is better suited for reproducibility; furthermore we release our method to generate RL compatibility training and test data from the original public data. 
% We believe this will serve as a useful benchmark for other RL related studies in the e-commerce context.


% talk about details of the two datasets, evaluation metrics, training setup, parameters, implementation in Tensorflow, and so on.

\subsubsection{Training Data Generation}
We collect 30 days of training data from our in-house search log. Table~\ref{tab:in-house-data} summarizes its basic statistics. The total number of examples in DIN-S (pre-RNN) training is 200m, while under the RNN/S3DDPG data format, we have 6m variable length sessions instead. While the majority of users only have a single session, the number of sessions per user can go as high as 100. This makes our knapsack session packing algorithm~\ref{alg:knapsack_rnn} a key step towards efficient training. 
\begin{table}[htbp]
\centering
\caption{In-house data statistics.}
\small
\begin{tabular}{c|c|c|c}
\hline
statistics & mean & minimum & maximum \\
\hline
Number of unique users & 3788232 & - & - \\
\hline
sessions per user &	13.42 & 1 & 113 \\
\hline
items per session & 26.97 & 1 & 499 \\
\hline
Features per (query, item) & 110 & - & - \\
\hline
\end{tabular}
\label{tab:in-house-data}
\end{table}

% The variance of number of items across different query sessions is quite high. This is characteristic of e-commerce search, which resembles recommendation streams more than web search. 
A characteristic of e-commerce search sessions is the huge variance in browsing depth (number of items in a session). In fact, some power user can browse content up to thousands of items within a single session. 
The short sessions (such as the minimum number of 2 items in the table) are due to lack of relevant results. 



% \subsubsection{Training Data Generation}
% For the DIN baseline training, we generate pointwise dataset from $N = 30$ days of search log. 
Each DIN-S training example consists of a single query and a single item under the query session. To leverage users' historic sequence information, the data also includes the item id, category id, shop id, and brand id of the historical sequence of clicked / purchased / carted items by the current user. The sequence is truncated at a maximum length of 500 for online serving efficiency. 

For RNN and S3DDPG, each example consists of a pair of items under the same query. In order to keep the training data compact, i.e., without expanding all possible item pairs, the training data adopts the User Session Input format (Section~\ref{subsubsec:data_format}). To ensure all sessions under a user are contained within each minibatch, and ordered chronologically, the session data is further sorted by session id as primary key and session timestamp as secondary key during the data generation mapreduce job.


% To further ensure each minibatch contains entire history of a user, the data is constructed so that sessions under the same user appear contiguously in the data. This is achieved by relying on sorting by the primary query key and secondary timestamp key in the mapreduce reducer phase. 

During training, a random pair of items is sampled from each session, with one positive label (purchased) and one negative label (viewed/clicked only). Thus each minibatch consists of $\sum_{u=1}^B |S_u|$ item pairs, where $S_u$ stands for the set of all sessions under user $u$ and $B$ is the minibatch size, in terms of number of users. 

\subsubsection{Offline Evaluation}
We evaluate all models on one day of search log data beyond the training period. For RRNN and S3DDPG, however, 
% the evluation set also includes the previous 29 days of data, for a total of $N = 30$ days. This is 
% To evaluate the baseline DIN-S model, we simply take one day of search log data beyond the training period and construct an evaluation set similar to training, that is, each example consists of a query and an item, with binary label being whether or not the item was purchased under that query.
% For the RNN and S3DDPG evaluation, 
% we construct the evaluation set in the User Session Input format similar to training. In particular, all sessions under a single user are ordered chronologically and continguously within the data set. in order to capture the historical information,
we also include $N-1$ days prior to the last day, for a total of $N = 30$ days. The first $29$ days are there to build the user state vector only. Their labels are needed for user state aggregation during RNN forward evolution. Only labels from the last day sessions are used in the evaluation metrics, to prevent any leakage between training and validation.
% Labels from earlier days are needed only for aggregation of the user states during the RNN forward evolution. 

\subsubsection{Offline Evaluation Metrics}
While cross entropy loss \eqref{eq:reward_definition} and square loss \eqref{eq:dqn_td_loss} are used during training of S3DDPG, for hold-out evaluation, we aim to assess the ability of the model to generalize forward in time. Furthermore even though the training is performed on sampled item pairs, in actual online serving, the objective is to optimize ranking for an entire session worth of items, whose number of can reach the hundreds. Thus we mainly look at session-wise metrics such as Session AUC or NDCG. Session AUC in particular is used to decide early stopping of model training: 

\begin{align} \label{eq:session_auc}
    \text{Session AUC}(\eta, \lambda) := \sum_{u = 1}^B \sum_{t = 1}^{|S_u|} \rm{AUC}(\eta_{u, t}, \lambda_{u, t}),
\end{align}
where $\eta_{u, t}$ denotes the list of model predictions for \textbf{all items} within the session $(u, t)$ and $\lambda_{u, t}$ the corresponding binary item purchase labels. This is in contrast with training, where $\eta_{u, t}$, $\lambda_{u, t}$ denote predictions and labels for a randomly chosen positive / negative item pair. 

The following standard definition of ROC AUC is used in \eqref{eq:session_auc} above. For two vectors $\boldsymbol{p}, \boldsymbol{t} \in \R^n$, where $t_i \in \{0, 1\}$:
\begin{align*}
\rm{AUC}(\boldsymbol{p}, \boldsymbol{t}) := \frac{\sum_{1 \leq i < j \leq n} \sign(p_i - p_j) \sign(t_i - t_j)}{n(n-1) / 2},
\end{align*}
where $\sign(x) = x / |x|$ for $x \neq 0$ and $\sign(0) = 0$.

% We systematically extract a model checkpoint that attains the highest session AUC among all saved checkpoints.

NDCG is another popular metric in search ranking, intended to judge full page result relevance \cite{distinguishability2013theoretical}. It again takes the model predictions (which can be converted into ranking positions) as well as corresponding labels for all items, and compute a position-weighted average of the label, normalized by its maximal possible value:
\begin{align*}
    \rm{NDCG}(\boldsymbol{p}, \boldsymbol{t}) = \sum_{i=1}^n \frac{2^{t_i} - 1}{\log_2(i + 1)} / \sum_{i=1}^{\sum_j t_j} \frac{2^{t_i} - 1}{\log_2(i + 1)}.
\end{align*}

% where $\rm{DCG}$ and $\rm{IDCG}$ are in turn defined by
% \begin{align}
% \rm{DCG}(\boldsymbol{p}, \boldsymbol{t}) &:= \sum_{i=1}^n \frac{2^{t_i} - 1}{\log_2(i + 1)} \\
% \rm{IDCG}(\boldsymbol{p}, \boldsymbol{t}) &:= \sum_{i \leq n: t_i = 1} \frac{2^{t_i} - 1}{\log_2(i + 1)}.
% \end{align}

\subsubsection{Online Metrics}
For e-commerce search, there are essentially three types of core online metrics. 
\begin{itemize}
    \item GMV stands for gross merchandise value, which measures the total revenue generated by a platform. Due to the variation of A/B bucket sizes, it is often more instructive to consider GMV per user.
    \item CVR stands for conversion rate and essentially measures the number of purchases per click. Again this is averaged over the number of users.
    \item CTR is simply click-through rate, which measures number of clicks per query request. We do not consider this metric in our online experiments since it is not directly optimized by our models.
\end{itemize}
% \subsubsection{Online Serving}
% The ultimate objective of introducing the sequential search context as well as reinforcement learning architecture is to promote better user experience and personalized result relevance, measured primarily through a set of core metrics such as conversion rate and GMV. Therefore model online serving is a crucial component of the overall evaluation.

% The serving of the baseline DIN model is straightforward. First the model gets loaded into the system. Then upon a query request from a given user, the search engine computes all the required features for all retrieved items under the query, and sends them to the DIN model. The bulk of the feature preparation and transmission lies in the item features (either 1-sided or jointly 2-sided with query and user information), as well as the user behaviorial sequence features, which however are capped at the length of 500. Once the scores are computed for all items, they are sent back to the search engine and sorted to produce a ranking among the retrieved results.

% RNN and S3DDPG models are served essentially identically. Therefore most of the serving infrastructure (Figure~\ref{fig:incremental_update}) has been built when we launched the RNN model. There are two major differences with the DIN or non-RNN types of models:
% \begin{itemize}
%     \item In addition to the regular input features required by the model, RNN models also receive a numeric vector for the previous user state. 
%     \item This user vector is updated in real time after every user query request, so that when the same user comes back next time, he or she gets served a model with an updated state vector.
% \end{itemize}
% The updating of the user vector takes the following two inputs
% \begin{itemize}
%     \item A list of state vector candidates returned by the model, one for each item scored.
%     \item The user's behavioral feedback upon viewing the ranked results in the search page; for our purpose, which items got purchased, if any. 
% \end{itemize}
% If no item was purchased within the previous query session, the user state stays the same. Otherwise it gets updated with the candidate state vector corresponding to the purchased item.

\subsection{Evaluation Results}


\begin{table}[htbp] 
\centering
\caption{Offline Metrics}
\begin{tabular}{c|c|c}
\hline
Model name & Session AUC & NDCG \\
\hline
DNN & 0.6765 & 0.5104 \\
DIN-S & 0.6875 & 0.5200 \\
RNN & 0.6915 & 0.5272 \\
S3DDPG & 0.6968 & 0.5307 \\
\hline
\end{tabular}
\label{tab:offline_metrics}
\end{table}
We present both Session AUC and NDCG for the 4 models listed in Table~\ref{tab:offline_metrics}. The DNN baseline simply aggregates the user sequential features through sum-pooling, all of which are id embeddings. The successive improvements are consistent between the two session-wise metrics: RNN improved upon DIN-S by about $0.4\%$ in Session AUC and $0.7\%$ in NDCG, while S3DDPG further improves upon RNN by another $0.5\%$ in Session AUC and $0.4\%$ in NDCG. The overall gain of S3DDPG is around a full $1\%$ in either metrics from the DIN-S baseline, and $2\%$ from the DNN baseline.


Table~\ref{tab:user_group_evaluation} highlights the gain of S3DDPG over the myopic RNN baseline on a variety of user subsets. For instance, along the dimension of users' past session counts, S3DDPG shows a significantly stronger performance for more seasoned users in both validation metrics. Another interesting dimension is whether the current query belongs to a completely new category of shopping intent compared to the users' past search experience. Users who issue such queries in the evaluation set are labeled ``Category New Users". Along that dimension, we see that S3DDPG clearly benefits more than RNN from similar queries searched in the past.

While there are a number of hyperparameters associated with reinforcement learning models in general, the most important one is arguably the discount factor $\gamma$ parameter. We choose $\gamma = 0.8$ for all our S3DDPG experiments, since we found little improvement when switching to other $\gamma$ value. Another important parameter specific to actor-critic style architecture is the relative weight $\mu$ between PG loss and TD loss. Interestingly, as we shift weight from TD to PG loss (increasing $\mu$), there is a noticeable trend of improvement in both AUC and NDCG, as shown in Figure~\ref{fig:hyperparameter}. This suggests the effectiveness of maximizing the long term cumulative reward directly, even at the expense of less strict enforcement of the Bellman equation through the TD loss. When $\mu$ is set to $1$, however, training degenerates, as the Q-value optimized by PG loss is not bound to the actual reward (cross entropy loss) any more.

\begin{figure}
    \centering
    %\includegraphics[width=0.9\linewidth]{SessionAUC_µ.png}
    \includegraphics[width=\linewidth]{mu.png}
    \caption{influence of hyperparameter $\mu$}
    \label{fig:hyperparameter}
\end{figure}

Finally we conduct 3 sets of online A/B tests, each over a timespan of 2 weeks. The overall metric improvements are reported in Table~\ref{tab:online_metrics}. The massive gain from DNN to DIN-S is expected, since the DNN baseline, with sum-pooling of the sequential features, is highly ineffective at using the rich source of sequential data. Nonetheless we also see modest to large improvements between RNN and DIN-S and between S3DDPG and RNN respectively, in all core business metrics. Figures~\ref{fig:daily_ucvr} present the daily UCVR metric comparison for the last 2 sets of A/B tests.  Aside from a single day of traffic variation, both RNN and S3DDPG show consistent improvement over their respective baselines. 
\begin{figure}
    \centering
%    \includegraphics[width=\linewidth]{UCVR-S3DDPG-RNN.png}
%     \caption{UCVR (conversion rate/unique user) delta in \% from DIN-S and RNN models over 14 days.}
%     \label{fig:rnn_v_DIN-S}
% \end{figure}
% \begin{figure}
%     \centering
    \includegraphics[width=\linewidth]{UCVR_ONLINE.png}
    \caption{Daily UCVR \% improvement for online A/B tests over 14 days.}
    \label{fig:daily_ucvr}
\end{figure}
% The gain from DIN to RNN is relatively easy to understand: by giving the model the full spectrum of input features from previous sessions in the near-term (30 days), RNN is equipped with much more context information about the user than the DIN model, which only gets a few categorical features of the past interacted items. 
% % The gain from RNN to S3DDPG is much more elusive. After all, they both have the same set of input features, and RNN, with its GRU kernel, is already a time-proven method for dealing with sequential data. Furthermore, the vast majority of users in the evaluation set only have a single session on the last day.

% The offline metrics gain from RNN to S3DDPG mainly comes from the removal of a weighting scheme used in both DIN and RNN, intended to promote items with higher prices, since besides user conversion rate, another important metric is GMV (gross merchandise volume), which measure the the total revenue generated by users' shopping activities on the search platform. While the price weighting scheme was very helpful in boosting GMV per user for the baseline DIN model as well as the RNN model, we found in online experiments that removing it did not cause any negative effect on GMV/user. Quite surprisingly, it in fact led to huge boost of both GMV/user as well as the closely related RPM (revenue-per-mil) metrics, both of which increased by nearly $2\%$ in relative term compared to RNN with price weighting, at a significance level of p-value $\leq 1\%$. 

% In fact, the trick lies in a technical detail mentioned earlier in Section~\ref{sec:method}. Namely, for both DIN and RNN, we introduced a weighting scheme to promote higher priced items within the search results. This was effective in boosting GMV and related revenue metrics, without sacrificing too much on click-through and conversion rate. For S3DDPG, however, this was removed. The hope was that reinforcement learning with its emphasis on long term reward is able to bring in more user conversion that would offset the short-term loss in per item revenue.

% Indeed from the online metrics Table~\ref{tab:online_metrics}, we see highly significant gains in GMV / user 


% As mentioned in Section~\ref{subsec:rnn:pairwise}, 

% Experiments to report:
% 1. DIN
% 2. RNN
% 3. DDPG:
% 3a. no target Q
% 3b. target Q
% 4. DQN: not convergent
% 5. 4 reward experiments
% 6. Analysis: long/short validation set
% 7. off-policy TopK
% 8. gamma grid search
% 9. TD + PG no tuning
% 10. target actor 



% \begin{table}[htbp]
% \centering
% \caption{Hyperparameter µ}
% \begin{tabular}{c|c|c}
% \hline
% Parameter & Session AUC & NDCG \\
% \hline
% 0 & -- & -- \\
% \hline
% 0.1 & 0.6887 & 0.5226 \\
% \hline
% 0.2 & 0.6946 & 0.5284 \\
% \hline
% 0.3 & 0.6939 & 0.5281 \\
% \hline
% 0.4 & 0.6941 & 0.5281 \\
% \hline
% 0.5 & 0.6968 & 0.5307 \\
% \hline
% 0.6 & 0.6959 & 0.5307 \\
% \hline
% 0.7 & 0.6970 & 0.5304 \\
% \hline
% 0.8 & 0.6979 & 0.5311 \\
% \hline
% 0.9 & 0.6985 & 0.5329 \\
% \hline
% 1.0 & -- & -- \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[htbp] \label{tab:offline_metrics}
% \centering
% \caption{S3DDPG vs RNN for Category New Users}
% \begin{tabular}{c|c|c|c}
% \hline
% Data Type & Model pairs & Session AUC & NDCG \\
% \hline
% New User & S3DDPG vs RNN & +0.3195\% & +0.1412\% \\
% \hline
% Old User & S3DDPG vs RNN & +0.6584\% & +0.6688\%\\
% \hline
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\centering
\caption{S3DDPG vs RNN for different user evaluation groups}
\begin{tabular}{c|c|c}
\hline
User Group  & Session AUC & NDCG \\
\hline
Past Session Count < 5  & +0.6534\% & +0.2418\% \\
Past Session Count >= 5  & +0.9544\% & +0.9092\%\\
Category New Users & +0.3195\% & +0.1412\% \\
Category Old Users & +0.6584\% & +0.6688\% \\
\hline
\end{tabular}
 \label{tab:user_group_evaluation}
\end{table}

\begin{table}[htbp]
\centering
\caption{Online Metrics}
\begin{tabular}{c|c|c|c}
\hline
Model pairs & GMV/user & CVR/user & RPM \\
\hline
DIN-S vs DNN & +4.05\%(1e-3) & +3.51\%(1e-3) & +4.08\%(5e-3) \\
RNN vs DIN-S & +0.60\%(5e-3) & +1.58\%(9e-3) & +0.49\%(8e-3) \\
S3DDPG vs RNN & +1.91\%(8e-3) & +0.78\%(1e-2) & +1.94\%(9e-3) \\
\hline
\end{tabular}
 \label{tab:online_metrics}
\end{table}
\vspace{-10pt}
% \begin{itemize}
% \item 离线实验指标
% \begin{itemize}
% \item RNN vs. DNN
% \begin{itemize}
% \item auc +0.94\%
% \end{itemize}
% \item DQN(gamma=0.8) vs. DNN
% \begin{itemize}
% \item auc +1.51\%
% \end{itemize}
% \end{itemize}
% \begin{itemize}
% \item DQN(gamma=0.8) vs. RNN
% \begin{itemize}
% \item auc +0.56\%
% \item results for other gamma 
% % (see Diagram~\ref{dia:gamma_sweep}
% \end{itemize}
% \end{itemize}
% \end{itemize}
% 在线实验指标
% \begin{itemize}
% \item RNN vs. DNN（线上观察7天）
% \begin{itemize}
% \item UV价值(搜索GMV/搜索用户) : +2.40\%
% \item UCVR(订单行/搜索用户): +3.09\%
% \item GMV: +1.99\%
% \item RPM(1000*搜索GMV/搜索量): +2.54\%
% \end{itemize}
% \item DDPG vs. RNN（线上观察7天）
% \begin{itemize}
% \item UV价值：+1.91\%
% \item UCVR：+0.78\%
% \item GMV：+1.77\%
% \item RPM：+1.94\%
% \item 流动性：+4.24\%
% \item 流动性: 使用rbo距离计算每个query今天的昨天TOP20 SKU排序的diff率，多天取平均。
% \item CID4基尼不纯度：0.95\%
% \item CID4基尼不纯度：TOP60坑位有曝光的CID4的gini不纯度
% \end{itemize}
% \item AB实验指标
% \end{itemize}


\label{sec:industrial}

% \subsection{Public Dataset Experiment}
% \label{sec:public}
% We take the Amazon review dataset as our starting point. Each reviewer is identified through his or her reviewer id. Since every review event contains a timestamp, we can naturally form a temporal sequence. Unlike our in-house dataset, however, there is no analogue of a session (with multiple items) in the dataset. Instead, we simply consider the sequence of review events. To take advantage of full recurrence as proposed, we include expensive features such as item titles, past reviews, etc, in addition to asin\_id (item id) and category names.

% \subsection{Case Study}
\label{sec:case}




==> DQN and DDPG in e-Commerce Search (5)/6-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We propose a previously unexplored class of machine learning problems, Sequential Search, that closely parallels Sequential Recommendation but comes with its own set of challenges and modeling requirements. We present three successively more advanced sequential models, DIN-S, RNN, and S3DDPG, to exploit the rich source of historical interactions between the user and the search platform. Practical techniques such as user session training data format, knapsack rearrangement of session sequence, and online incremental serving are discussed extensively. Finally systematic offline experiments on a large scale industrial dataset are performed, showing significant incremental improvement between all successive model pairs. These results are further validated with substantial gains in online A/B tests, showing that principled modeling of users' sequential behavior information can significantly improve user experience and personalized search relevance.
% modeling approach to leveraging users' sequential information can translate into massive business revenue jumps.


% We present a comprehensive modeling framework to incorporate elements of reinforcement learning into the personalized e-commerce search system. We demonstrate massive improvements from the DNN to RNN, as well as from RNN to DPPG. The latter exhibits long term user engagement improvements, as well as significant gains in result diversity and personalization coverage. The use of specialized data structure and RNN input optimization facilitate efficient training. By updating the user state daily, the model is trained at a relatively low frequency (weekly) while still retains the latest user information, thus is capable of handling much larger data/model size than a non-sequential network structure.

